A Quantum of QUIC: Dissecting Cryptography with Post-Quantum Insights

QUIC is a new network protocol standardized in 2021. It was designed to replace the TCP/TLS stack and is based on UDP. The most current web standard HTTP/3 is specifically designed to use QUIC as transport protocol. QUIC claims to provide secure and fast transport with low-latency connection establishment, flow and congestion control, reliable delivery, and stream multiplexing. To achieve the security goals, QUIC enforces the usage of TLS 1.3. It uses authenticated encryption with additional data (AEAD) algorithms to not only protect the payload but also parts of the header. The handshake relies on asymmetric cryptography, which will be broken with the introduction of powerful quantum computers, making the use of post-quantum cryptography inevitable. This paper presents a detailed evaluation of the impact of cryptography on QUIC performance. The high-performance QUIC implementations LSQUIC, quiche, and MsQuic are evaluated under different aspects. We break symmetric cryptography down to the different security features. To be able to isolate the impact of cryptography, we implemented a NOOP AEAD algorithm which leaves plaintext unaltered. We show that QUIC performance increases by 10 to 20% when removing packet protection. The header protection has negligible impact on performance, especially for AES ciphers. We integrate post-quantum cryptographic algorithms into QUIC, demonstrating its feasibility without major changes to the QUIC libraries by using a TLS library that implements post-quantum algorithms. Kyber, Dilithium, and FALCON are promising candidates for post-quantum secure QUIC, as they have a low impact on the handshake duration. Algorithms like SPHINCS+ with larger key sizes or more complex calculations significantly impact the handshake duration and cause additional issues in our measurements.

==> acronyms.tex <==

\DeclareAcronym{cpu}{
    short               = {CPU},
    long                = {CPU}, % we dont need this as long
    first-style         = short,
}

\DeclareAcronym{ack}{
    short               = {ACK},
    long                = {acknowledgment},
}

\DeclareAcronym{aes}{
    short               = {AES},
    long                = {Advanced Encryption Standard},
}

\DeclareAcronym{aesni}{
    short               = {AES-NI},
    long                = {Advanced Encryption Standard},
    first-style         = short,
}

\DeclareAcronym{chacha20}{
    short               = {ChaCha20},
    long                = {ChaCha20},
    first-style         = short,
}

\DeclareAcronym{qir}{
	short				= {QIR},
	long				= {QUIC Interop Runner},
}

\DeclareAcronym{io}{
    short               = {I/O},
    long                = {I/O},% we dont need this as long
    first-style         = short,
}


\DeclareAcronym{udp}{
	short				= {UDP},
	long				= {UDP}, % we dont need this as long
	first-style			= short,
}

\DeclareAcronym{tcp}{
    short               = {TCP},
    long                = {TCP}, % we dont need this as long
    first-style         = short,
}


\DeclareAcronym{dpdk}{
    short               = {DPDK},
    long                = {Data Plane Development Kit},
}

\DeclareAcronym{tls}{
    short               = {TLS},
    long                = {Transport Layer Security},
    first-style         = short,
}

\DeclareAcronym{aead}{
    short               = {AEAD},
    long                = {authenticated encryption with additional data},
}


\DeclareAcronym{ietf}{
    short               = {IETF},
    long                = {Internet Engineering Task Force},
}

\DeclareAcronym{http}{
    short               = {HTTP},
    long                = {Hypertext Transfer Protocol},
    first-style         = short,
}

\DeclareAcronym{https}{
    short               = {HTTPS},
    long                = {Hypertext Transfer Protocol Secure},
    first-style         = short,
}

\DeclareAcronym{nic}{
    short               = {NIC},
    long                = {Network Interface Card},
}

\DeclareAcronym{dma}{
    short               = {DMA},
    long                = {Direct Memory Access},
}


\DeclareAcronym{tso}{
    short               = {TSO},
    long                = {TCP Segmentation Offload},
}

\DeclareAcronym{lro}{
    short               = {LRO},
    long                = {Large Receive Offload},
}

\DeclareAcronym{gso}{
    short               = {GSO},
    long                = {Generic Segmentation Offload},
}

\DeclareAcronym{gro}{
    short               = {GRO},
    long                = {Generic Receive Offload},
}

\DeclareAcronym{mss}{
    short               = {MSS},
    long                = {Maximum Segment Size},
}

\DeclareAcronym{nat}{
    short               = {NAT},
    long                = {Network Address Translation},
}

\DeclareAcronym{sctp}{
    short               = {SCTP},
    long                = {Stream Control Transmission Protocol},
}

\DeclareAcronym{rcvbuf}{
    short               = {RCVBUF},
    long                = {Receive Buffer},
}

\DeclareAcronym{sndbuf}{
    short               = {SNDBUF},
    long                = {Send Buffer},
}

\DeclareAcronym{cc}{
    short               = {CC},
    long                = {Congestion Control},
}

\DeclareAcronym{os}{
    short               = {OS},
    long                = {Operating System},
}

\DeclareAcronym{mtu}{
    short               = {MTU},
    long                = {Maximum Transmission Unit},
}

\DeclareAcronym{ecb}{
    short               = {ECB},
    long                = {Electronic Code Book},
}

\DeclareAcronym{oqs}{
    short               = {OQS},
    long                = {Open Quantum Safe},
}

\DeclareAcronym{pqc}{
    short               = {PQC},
    long                = {post-quantum cryptography},
}

\DeclareAcronym{ttfb}{
    short               = {TTFB},
    long                = {Time To First Byte},
}

\DeclareAcronym{nist}{
    short               = {NIST},
    long                = {National Institute of Standards and Technology},
}

\DeclareAcronym{kem}{
    short               = {KEM},
    long                = {key encapsulation mechanism},
}

\DeclareAcronym{masque}{
    short               = {MASQUE},
    long                = {Multiplexed Application Substrate over QUIC Encryption},
    first-style         = short,
}

\DeclareAcronym{rtt}{
    short               = {RTT},
    long                = {Round-Trip Time},
    first-style         = short,
}

\DeclareAcronym{SHA}{
    short               = {SHA},
    long                = {SHA},
    first-style         = short,
}
\DeclareAcronym{BIKE}{
    short               = {BIKE},
    long                = {BIKE},
    first-style         = short,
}
\DeclareAcronym{HQC}{
    short               = {HQC},
    long                = {HQC},
    first-style         = short,
}
\DeclareAcronym{CRYSTALS}{
    short               = {CRYSTALS},
    long                = {CRYSTALS},
    first-style         = short,
}
\DeclareAcronym{RSA}{
    short               = {RSA},
    long                = {RSA},
    first-style         = short,
}
\DeclareAcronym{FALCON}{
    short               = {FALCON},
    long                = {FALCON},
    first-style         = short,
}

